SideControl: Controlled Open-domain Dialogue Generation via Additive Side Networks

Transformer-based pre-trained language models boost the performance of open-domain dialogue systems. Prior works leverage Transformer-based pre-trained language models to generate texts with desired attributes in two general approaches: (1) gradient-based methods: updating all latent representations of pre-trained models with gradients from attribute models; (2) weighted-decoding methods: re-ranking beam candidates from pre-trained models with attribute functions. However, gradient-based methods lead to high computation cost and can easily get overfitted on small training sets, while weighted-decoding methods are inherently constrained by the low-variance high-bias pre-trained model. In this work, we propose a novel approach to control the generation of Transformer-based pre-trained language models: the SideControl framework, which leverages a novel control attributes loss to incorporate useful control signals, and is shown to perform well with very limited training samples. We evaluate our proposed method on two benchmark open-domain dialogue datasets, and results show that the SideControl framework has better controllability, higher generation quality and better sample-efficiency than existing gradient-based and weighted-decoding baselines.

==> Makefile <==
### latex.makefile
# Author: Jason Hiebel

PROJECT = main

# This is a simple makefile for compiling LaTeX documents. The core assumption
# is that the resulting documents should have any parameters effecting
# rendering quality set to theoretical limits and that all fonts should be
# embedded. While typically overkill, the detriment to doing so is negligible.

# Targets:
#    default : compiles the document to a PDF file using the defined
#              latex generating engine. (pdflatex, xelatex, etc)
#    display : displays the compiled document in a common PDF viewer.
#              (currently linux = evince, OSX = open)
#    clean   : removes the obj/ directory holding temporary files

default: obj/$(PROJECT).pdf

display: default
	(${PDFVIEWER} obj/$(PROJECT).pdf &)


### Compilation Flags
PDFLATEX_FLAGS  = -halt-on-error -output-directory obj/

TEXINPUTS = .:obj/
TEXMFOUTPUT = obj/


### File Types (for dependancies)
TEX_FILES = $(shell find . -name '*.tex' -or -name '*.sty' -or -name '*.cls')
BIB_FILES = $(shell find . -name '*.bib')
BST_FILES = $(shell find . -name '*.bst')
IMG_FILES = $(shell find . -path '*.jpg' -or -path '*.png' -or \( \! -path './obj/*.pdf' -path '*.pdf' \) )


### Standard PDF Viewers
# Defines a set of standard PDF viewer tools to use when displaying the result
# with the display target. Currently chosen are defaults which should work on
# most linux systems with GNOME installed and on all OSX systems.

UNAME := $(shell uname)

ifeq ($(UNAME), Linux)
PDFVIEWER = evince
endif

ifeq ($(UNAME), Darwin)
PDFVIEWER = open
endif


### Clean
# This target cleans the temporary files generated by the tex programs in
# use. All temporary files generated by this makefile will be placed in obj/
# so cleanup is easy.

clean::
	rm -rf obj/

### Core Latex Generation
# Performs the typical build process for latex generations so that all
# references are resolved correctly. If adding components to this run-time
# always take caution and implement the worst case set of commands.
# Example: latex, bibtex, latex, latex
#
# Note the use of order-only prerequisites (prerequisites following the |).
# Order-only prerequisites do not effect the target -- if the order-only
# prerequisite has changed and none of the normal prerequisites have changed
# then this target IS NOT run.
#
# In order to function for projects which use a subset of the provided features
# it is important to verify that optional dependancies exist before calling a
# target; for instance, see how bibliography files (.bbl) are handled as a
# dependency.

obj/:
	mkdir -p obj/

obj/$(PROJECT).aux: $(TEX_FILES) $(IMG_FILES) | obj/
	pdflatex $(PDFLATEX_FLAGS) $(PROJECT)

obj/$(PROJECT).bbl: $(BIB_FILES) | obj/$(PROJECT).aux
	bibtex obj/$(PROJECT)
	pdflatex $(PDFLATEX_FLAGS) $(PROJECT)

obj/$(PROJECT).pdf: obj/$(PROJECT).aux $(if $(BIB_FILES), obj/$(PROJECT).bbl)
	pdflatex $(PDFLATEX_FLAGS) $(PROJECT)
	grep -e "Warning" --color auto obj/$(PROJECT).log


==> ethical.tex <==
\section{Ethical Considerations}
The goal of this work is to control attributes generation of the Transformer-based language models.
To guarantee the reproducibility of this work, we provide essential details in the main content and the appendices.
Although the proposed controlled generation method does not directly involve any ethical issues, the pre-trained language models could generate some texts which may lead to some ethical concerns, such as some offensive or toxic responses.
Additional techniques are needed to address these issues, for example, filtering out some toxic words from the vocabulary during text prepossessing.

